Exploring the Impact of Corpus Diversity on Financial Pretrained Language Models

Over the past few years, various domain-specific pretrained language models (PLMs) have been proposed and have outperformed general-domain PLMs in specialized areas such as biomedical, scientific, and clinical domains. In addition, financial PLMs have been studied because of the high economic impact of financial data analysis. However, we found that financial PLMs were not pretrained on sufficiently diverse financial data. This lack of diverse training data leads to a subpar generalization performance, resulting in general-purpose PLMs, including BERT, often outperforming financial PLMs on many downstream tasks. To address this issue, we collected a broad range of financial corpus and trained the Financial Language Model (FiLM) on these diverse datasets. Our experimental results confirm that FiLM outperforms not only existing financial PLMs but also general domain PLMs. Furthermore, we provide empirical evidence that this improvement can be achieved even for unseen corpus groups.

==> related_works.tex <==
\section{Related Works}
% 빼거나 맨뒤 혹은 appendix
To adopt a PLM to a specific domain, it is necessary to pretrain the model using a corpus that is relevant to that domain.
It has been demonstrated to perform well and has been widely applied in various fields.
There are well-known studies like  BioBERT~\cite{lee2020biobert}, ClinicalBERT~\cite{alsentzer2019publicly}, and SciBERT~\cite{beltagy2019scibert}, which have been proven through experiments conducted by the \citet{gururangan-etal-2020-dont}.

Similarly, domain-specific PLM research has been applied in financial NLP.
Pre-training on the financial corpus demonstrates outperforming on financial tasks.
There are established studies known as FinBERT a total of three papers.
All of which are pre-trained Language Models trained on Financial Corpora.
% citation paper 이름으로만 작성하기. 
\finA pre-trained on the TRC2-financial corpus comprising Reuters news articles.
\finY pre-trained using data from Edgar Filings, Earning Call Transcripts, and Analyst Reports.
In \finL, the pre-trained corpus consists of FinWeb, Yahoo Finance, and Reddit Finance QA.
The information about the data and tasks used in training FinBERT models is provided in Appendix~%\ref{}.

There are various types of text data, leading to a diverse set of tasks.
Some prominent tasks in the financial domain include sentiment analysis~\cite{malo2014good}, named entity recognition~\cite{alvarado2015domain}. 
Additionally, the \citet{shah2022flue} has introduced various financial task benchmarks.
Recently, new tasks have also been explored. FiNER~\cite{loukas2022finer}, for example, introduced a task that utilizes XBRL tagging to identify numerical types.
FinQA~\cite{chen2021finqa} also developed a Question Answering task by leveraging SEC filings reports. We provide a detailed introduction to the tasks in Section~§\ref{subsec:tasks_dataset}.



